Lower bounds on information complexity via zero-communication protocols and applications

We show that almost all known lower bound methods for communication complexity are also lower bounds for the information complexity. In particular, we define a relaxed version of the partition bound of Jain and Klauck and prove that it lower bounds the information complexity of any function. Our relaxed partition bound subsumes all norm based methods (e.g. the factorization norm method) and rectangle-based methods (e.g. the rectangle/corruption bound, the smooth rectangle bound, and the discrepancy bound), except the partition bound. Our result uses a new connection between rectangles and zero-communication protocols where the players can either output a value or abort. We prove the following compression lemma: given a protocol for a function f with information complexity I, one can construct a zero-communication protocol that has non-abort probability at least 2^{-O(I)} and that computes f correctly with high probability conditioned on not aborting. Then, we show how such a zero-communication protocol relates to the relaxed partition bound. We use our main theorem to resolve three of the open questions raised by Braverman. First, we show that the information complexity of the Vector in Subspace Problem is {\Omega}(n^{1/3}), which, in turn, implies that there exists an exponential separation between quantum communication complexity and classical information complexity. Moreover, we provide an {\Omega}(n) lower bound on the information complexity of the Gap Hamming Distance Problem.

==> appx.tex <==
\section{Relaxed partition bound and other bounds}\label{app:bprt}
Recall the definition of the partition bound $\prt_\eps(f)$ in~\cite{JK10}:
\begin{definition}[\cite{JK10}]
The partition bound $\prt_\eps(f)$ is defined as the value of the following linear program:
%  \begin{enumerate}
%  \item Primal form:
\begin{align}
\prt_\eps(f)=\min_{w_{R,z}\geq 0}  \sum_{R,z} w_{R,z} \quad \text{ subject to:}\quad
 &\forall (x,y)\in \setin,\quad \sum_{R:(x,y)\in R} w_{R,f(x,y)} \geq 1-\eps\quad \nonumber\\
 &\forall (x,y)\in\calX\times\calY,\quad \sum_{z,R:(x,y)\in R} w_{R,z} =1
\end{align}
%  \item Dual form:
% \begin{align}
% \prt_\eps(f)=\max_{v_{x,y}\geq 0, w_{x,y}} & \sum_{(x, y)\in \setin} (1 - \eps) v_{x, y} -
%   \sum_{(x, y)} w_{x,y} \text{ subject
%     to:} \nonumber\\
% \forall R,b, & \quad \sum_{(x, y) \in R \cap f^{-1}(b)}
% v_{x,y} - \sum_{(x, y) \in R}w_{x,y} \leq 1
% \end{align}
% \end{enumerate}
\end{definition}

We first show that $\bprt_\eps(f)$ is indeed a relaxation of the partition bound by providing linear programming formulations for $\bprt_\eps^\mu(f)$ and $\bprt_\eps(f)$.
\begin{claim}\label{claim:bprt-lp}
$\bprt_\eps^\mu(f)$ can be expressed as the following linear programs:
\begin{enumerate}
 \item Primal form:
\begin{align}
\bprt_\eps^\mu(f)=\min_{w_{R,z}\geq 0} & \sum_{R,z} w_{R,z} \quad \text{ subject to:}
\nonumber\\
 & \sum_{(x,y)\in \setin}\mu_{x,y}\sum_{R:(x,y)\in R} w_{R,f(x,y)}+\sum_{(x,y)\notin \setin}\mu_{x,y}\sum_{z,R:(x,y)\in R} w_{R,z} \geq 1-\eps \nonumber\\
 &\forall (x,y)\in\calX\times\calY,\quad \sum_{z,R:(x,y)\in R} w_{R,z} \leq 1
\end{align}
 \item Dual form:
\begin{align}
\bprt_\eps^\mu(f)=\max_{\alpha\geq 0, \beta_{x,y}\geq 0} & (1 - \eps)\alpha +
  \sum_{(x, y)\in\calX\times\calY} \beta_{x,y} \text{ subject
    to:} \nonumber\\
\forall R,z, & \quad \sum_{(x, y) \in R \cap f^{-1}(z)}
\alpha\mu_{x,y} + \sum_{(x, y) \in R \setminus \setin}
\alpha\mu_{x,y} - \sum_{(x, y) \in R}\beta_{x,y} \leq 1
\end{align}
\end{enumerate}
Similarly, $\bprt_\eps(f)$ is given by the value of the following linear programs:
\begin{enumerate}
 \item Primal form:
\begin{align}
\bprt_\eps(f)=\min_{w_{R,z}\geq 0}  \sum_{R,z} w_{R,z} \quad \text{ subject to:}\quad
 &\forall (x,y)\in \setin,\quad \sum_{R:(x,y)\in R} w_{R,f(x,y)} \geq 1-\eps \nonumber\\
 &\forall (x,y)\notin \setin,\quad \sum_{z,R:(x,y)\in R} w_{R,z} \geq 1-\eps \nonumber\\
 &\forall (x,y)\in\calX\times\calY,\quad \sum_{z,R:(x,y)\in R} w_{R,z} \leq 1
\end{align}
 \item Dual form:
\begin{align}
\bprt_\eps(f)=\max_{\alpha_{x,y}\geq 0, \beta_{x,y}\geq 0} & \sum_{(x, y)\in\calX\times\calY} (1 - \eps) \alpha_{x,y} -
  \sum_{(x, y)\in\calX\times\calY} \beta_{x,y} \text{ subject
    to:} \nonumber\\
\forall R,z, & \quad \sum_{(x, y) \in R \cap f^{-1}(z)} \alpha_{x,y} + \sum_{(x, y) \in R \setminus \setin}
\alpha_{x,y} - \sum_{(x, y) \in R}\beta_{x,y} \leq 1
\end{align}
\end{enumerate}
\end{claim}
\begin{proof}
The primal form of $\bprt_\eps^\mu(f)$ can be obtained from \autoref{def:relaxed-prt} by using the change of variables $w_{R,z}=p_{R,z}/\eta$. The dual form then follows from standard linear programming duality.

As for $\bprt_\eps(f)$, by \autoref{def:relaxed-prt} we have $\bprt_\eps(f)=\max_\mu\bprt_\eps^\mu(f)$. The dual form of $\bprt_\eps(f)$ then follows from the dual form of $\bprt_\eps^\mu$ via the change of variables $\alpha_{x,y}=\alpha\mu_{x,y}$. Finally, the primal form can be obtained via standard linear programming duality.
\end{proof}
Let us compare the primal form of $\bprt_\eps(f)$ with the definition of the partition bound $\prt_\eps(f)$. We see that the first two constraints in $\bprt_\eps(f)$ imply that $\sum_{z,R:(x,y)\in R} w_{R,z}$ lies between $1-\eps$ and $1$, while for $\prt_\eps(f)$, this should be exactly equal to $1$.  In terms of zero-communication protocols, this difference can be interpreted as follows: for $\prt_\eps(f)$, the protocol should output anything but $\bot$ with constant probability $\eta$ for any input $x,y$, while for $\bprt_\eps(f)$, the probability of not outputting $\bot$ is allowed to fluctuate between $(1-\eps)\eta$ and $\eta$.

Just as the partition bound, the relaxed partition bound is stronger than the smooth rectangle bound, defined in~\cite{JK10} as follows:
\begin{definition}[\cite{JK10}] The smooth rectangle bound $\srec_\eps^{z_0}(f)$ is the value of the following linear program:
\begin{align}
\srec_\eps^{z_0}(f)=\min_{w'_{R}\geq 0}  \sum_{R} w'_{R} \quad \text{ subject to:}\quad
 &\forall (x,y)\in f^{-1}(z_0),\quad \sum_{R:(x,y)\in R} w'_{R} \geq 1-\eps \nonumber\\
 &\forall (x,y)\in f^{-1}(z_0),\quad \sum_{R:(x,y)\in R} w'_{R} \leq 1 \nonumber\\
 &\forall (x,y)\in \setin\setminus f^{-1}(z_0),\quad \sum_{R:(x,y)\in R} w'_{R} \leq \eps.
\end{align}
\end{definition}

Let us now prove \autoref{claim:srec-bprt-prt}, that is,  $\srec^{z_0}_\eps(f)\leq \bprt_\eps(f)\leq\prt_\eps(f)$

\begin{proof}[Proof of \autoref{claim:srec-bprt-prt}]
 The second inequality is immediate since the only difference between the linear programs is that the constraint $\sum_{z,R:(x,y)\in R} w_{R,z} =1$ in the primal form of $\prt_\eps(f)$ has been relaxed to $1-\eps\leq\sum_{z,R:(x,y)\in R} w_{R,z} \leq 1$.

As for the first inequality, let $w_{R,z}$ be an optimal solution for the primal formulation of $\bprt_\eps(f)$ in \autoref{claim:bprt-lp}. Then, it is straightforward to check that setting $w'_R=w_{R,z_0}$ leads to a feasible point for $\srec_\eps^{z_0}(f)$, with objective value $\sum_{R} w'_{R}=\sum_R w_{R,z_0}\leq \sum_{R,z} w_{R,z}=\bprt_\eps(f)$.
\end{proof}


% \section{Rectangle bound}
% 
% Jain and Klauck give the following dual formulation for the rectangle bound.
% \begin{align}
% \rec_\eps^b(f) = \text{maximize } & \sum_{(x, y) \in f^{-1}(b)} (1 - \eps) v_{x, y} -
%   \sum_{(x, y) \in f^{-1}(1-b)} \eps v_{x,y} \text{ subject
%     to:} \label{eq:dualobj} \\
% \forall R, & \quad \sum_{(x, y) \in f^{-1}(b) \cap R}
% v_{x,y} - \sum_{(x, y) \in f^{-1}(1-b) \cap R}v_{x,y} \leq 1 \\
% \forall x, y, & \quad v_{x,y} \geq 0
% \end{align}
% 
% In the distributional case, Jain and Klauck give the following \textit{natural} definition of the distributional rectangle bound~\cite{JK10}.
% \begin{align*}
% \widetilde{\rec}_\eps^{b,\mu}(f)=\min_{R} \frac{1}{\mu(R\cap f^{-1}(b))} \quad \text{ subject to:}
% \quad \eps \mu(R\cap f^{-1}(b))\geq \mu(R\cap f^{-1}(\bar{b})).
% \end{align*}
% 
% Both versions are close to each other (the proofs of all claims in this section are provided in \autoref{app:proofs-preliminaries}):
% 
% \begin{claim}\label{claim:dis-rec-close}
%  $\frac{1-\eps}{4}\widetilde{\rec}_{2\eps/(1-\eps)}^{b,\mu}(f)\leq \rec_\eps^{b,\mu}(f)\leq\frac{1}{2}\widetilde{\rec}_\eps^{b,\mu}(f)$.
% \end{claim}
% 
% 
% From Claim~\ref{claim:dis-rec-close}, both definitions of the smooth rectagle bound
% are equivalent:
% \begin{claim}
%  $\frac{1-\eps}{4}\widetilde{\srec}_{2\eps/(1-\eps),\delta}^{b,\mu}(f)\leq \srec_{\eps,\delta}^{b,\mu}(f)\leq\frac{1}{2}\widetilde{\srec}_{\eps,\delta}^{b,\mu}(f)$.
% \end{claim}
% 
% %\section{Proof of Claims from \autoref{sec:preliminaries}}\label{app:proofs-preliminaries}
% \begin{proof}[Proof of~\autoref{claim:dis-rec-close}]
% For the second inequality, let $R_0$ be a rectangle achieving $\widetilde{\rec}_\eps^{b,\mu}(f)=\eta^{-1}$, with $\eta=\mu(R_0\cap f^{-1}(b))$. By definition, we have $\mu(R\cap f^{-1}(\bar{b}))\leq \eps \eta$, therefore the distribution $p_R=\delta_{RR_0}$ is a feasible point for $\rec_\eps^{b,\mu}(f)$, witnessing that $\rec_\eps^{b,\mu}(f)\leq 1/(2\eta)=\widetilde{\rec}_\eps^{b,\mu}(f)/2$.
% 
% For the first inequality, let $p_R$ be a distribution minimizing the linear program for $\rec_\eps^{b,\mu}(f)=1/(2\eta)$. In the following, we will denote by $\Exp[\cdot]$ the expectation over $R$ distributed according to $p_R$. Let $\eps'=\eps/(1-\eps)$, so that
% \begin{align*}
%  \eps' \Exp[\mu(R\cap f^{-1}(b))]\geq \Exp[\mu(R\cap f^{-1}(\bar{b}))]
% \end{align*}
% Let $M=\Exp[\mu(R\cap f^{-1}(b))]$. Since $\mu(R)=\mu(R\cap f^{-1}(b))+\mu(R\cap f^{-1}(\bar{b}))$, we have $(1+\eps') M\geq \Exp[\mu(R)]$.
% 
% Let us partition the set of rectangles $R$ such that $p_R\neq 0$ into two subsets, a set of \textit{large} rectangles $S_+$ and a set of \textit{small} rectangles $S_-$ (these will be defined more precisely later). By abuse of notation, we denote by $S_+$ the event $R\in S_+$, and similarly for $S_-$.
% Let $p_+=\sum_{R\in S_+} p_R$, $p_-=\sum_{R\in S_-} p_R$, $M_+=\Exp[\mu(R\cap f^{-1}(b))|S_+]$ and $M_-=\Exp[\mu(R\cap f^{-1}(b))|S_-]$, and note that $p_+M_++p_-M_-=M$.
% 
% Let us now choose some constant $0\leq\alpha\leq 1$ and split the rectangles between $S_+$ and $S_-$ so that $\mu(R\cap f^{-1}(b))\geq\alpha$ for all $R\in S_+$, $\mu(R\cap f^{-1}(b))\leq\alpha$ for all $R\in S_-$, and $p_+M_+=p_-M_-=M/2$ (this is always possible by choosing the right constant $\alpha$ and distributing the rectangles such that $\mu(R\cap f^{-1}(b))=\alpha$ appropriately between $S_+$ and $S_-$).
% 
% Recall that $(1+\eps') M\geq \Exp[\mu(R)]$, therefore
% \begin{align*}
%  (1+\eps') (p_+M_++p_-M_-)&\geq p_+ \Exp[\mu(R)|S_+]+p_-\Exp[\mu(R)|S_-]\\
% \Leftrightarrow (1+\eps') M_+&\geq \Exp[\mu(R)|S_+] + \frac{p_-}{p_+}(\Exp[\mu(R)|S_-]-(1+\eps')M_-)\\
% &\geq \Exp[\mu(R)|S_+] -\eps' \frac{p_-}{p_+} M_-,
% \end{align*}
% where we have used the fact that $\Exp[\mu(R)|S_-]\geq \Exp[\mu(R\cap f^{-1}(b))|S_-]= M_- $. Moreover, since $p_+M_+=p_-M_-$, we have
% \begin{align*}
% (1+\eps') M_+&\geq \Exp[\mu(R)|S_+]-\eps' M_+\\
% \Leftrightarrow (1+2\eps') M_+ &\geq \Exp[\mu(R)|S_+].
% \end{align*}
% Therefore, by definition of $M_+$, there must exist a rectangle $R\in S_+$ such that
% \begin{align}
%  (1+2\eps') \mu(R\cap f^{-1}(b))&\geq \mu(R)\\
% \Leftrightarrow 2\eps' \mu(R\cap f^{-1}(b))&\geq \mu(R\cap f^{-1}(\bar{b}))
% \end{align}
% Since $R\in S_+$, this rectangle satisfies $\mu(R\cap f^{-1}(b))\geq\alpha$, and therefore constitutes a witness that $\widetilde{\rec}_{2\eps'}^{b,\mu}(f)\leq 1/\alpha$. Finally, note that $\alpha\geq M_-\geq p_- M_-=M/2$ and $M\geq(1-\eps)\eta$, hence $\widetilde{\rec}_{2\eps'}^{b,\mu}(f)\leq 2/M\leq 2/((1-\eps)\eta)=(4/(1-\eps))\rec_\eps^{b,\mu}(f)$.
% \end{proof}
% 
% 
% Jain and Klauck give the following \textit{natural} definition for the distributional smooth-rectangle bound~\cite{JK10}:
% \begin{align*}
%   \widetilde{\srec}_{\eps,\delta}^{b,\mu}(f)=\max\{\widetilde{\rec}_\eps^{b,\mu}(g):\Pr_{(x,y)\leftarrow\mu}[f(x,y)\neq g(x,y)]<\delta;\mu(g^{-1}(b))\geq1/2\}.
% \end{align*}
% 
% In the next proofs, we will use the fact that $\rec_\eps^{b,\mu}(f)$ can be expressed as the following linear programs (this follows from the change of variable $w_R=p_R/(2\eta)$ for the primal, and from standard linear programming duality for the dual):
% \begin{enumerate}
%  \item Primal form:
% \begin{align}\label{eq:rec-primal}
% \rec_\eps^{b,\mu}(f)=\min_{w_R\geq 0}  \sum_R w_R \quad \text{ subject to:}\quad 
%  &\sum_R   \mu(R\cap f^{-1}(b)) w_R \geq \frac{1 - \eps}{2} \nonumber\\
%  &\sum_R   \mu(\cap f^{-1}(\bar{b}))w_R \leq \frac{\eps}{2}
% \end{align}
% \item Dual form
% \begin{align}\label{eq:rec-dual}
% \rec_\eps^{b,\mu}(f)=\max_{\alpha\geq 0,\beta\geq 0} & \alpha (1 - \eps) -
%   \beta \eps \text{ subject
%     to:} \nonumber\\
% \forall R, & \quad \mu( R\cap f^{-1}(b))
% \alpha - \mu( R\cap f^{-1}(\bar{b})) \beta \leq \frac{1}{2}
% \end{align}
% \end{enumerate}
% 
% \begin{proof}[Proof of~\autoref{claim:non-dist-rec}]
% Let us consider the dual form~(\ref{eq:rec-dual}) of the linear program for $\rec_\eps^{b,\mu}(f)$.
% Maximizing over a distribution $\mu$ such that $\mu(f^{-1}(b))\geq 1/2$, we obtain the following program:
% \begin{align}\label{eq:lp-dist-rec}
% \max_{\alpha\geq 0,\beta\geq 0,\mu_{x,y}\geq 0} & \alpha (1 - \eps) -
%   \beta \eps \text{ subject
%     to:}\\
% \forall R, & \quad  \mu(R \cap f^{-1}(b))
% \alpha - \mu( R\cap f^{-1}(\bar{b})) \beta \leq \frac{1}{2}\nonumber\\
% &\sum_{x,y\in f^{-1}(b)}\mu_{x,y}\geq \frac{1}{2}\nonumber\\
% &\sum_{x,y}\mu_{x,y}=1\nonumber
% \end{align}
% 
% Let us first prove that $\max\{\rec_\eps^{b,\mu}(f):\mu(f^{-1}(b))\geq1/2\}\geq\rec_\eps^{b}(f)$.
% Starting from an optimal point of the dual linear program for $\rec_\eps^{b}(f)$, we construct a feasible point for~(\ref{eq:lp-dist-rec}) by setting
% \begin{align*}
%  \alpha&=\sum_{(x, y) \in f^{-1}(b)}v_{x,y}, &
%  \beta&=\sum_{(x, y) \in f^{-1}(\bar{b})}v_{x,y}.
% \end{align*}
% We note that $\alpha>0$ since we must have $\rec_\eps^{b}(f)>0$, and then choose the distribution $\mu$ as follows: for $(x,y)\in f^{-1}(b)$, we take $\mu_{x,y}=v_{x,y}/(2\alpha)$; for $(x,y)\in f^{-1}(\bar{b})$, we take $\mu_{x,y}=v_{x,y}/(2\beta)$ if $\beta\neq 0$, and arbitrarily such that $\mu(f^{-1}(\bar{b}))=1/2$ if $\beta=0$. This is indeed a feasible point for~(\ref{eq:lp-dist-rec}), and achieves the same objective value as the optimal point of $\rec_\eps^{b}(f)$, hence $\max\{\rec_\eps^{b,\mu}(f):\mu(f^{-1}(b))\geq1/2\}\geq\rec_\eps^{b}(f)$.
% 
% For the other direction, we consider an optimal point of~(\ref{eq:lp-dist-rec}), and construct a feasible point for $\rec_\eps^{b}(f)$ by setting $v_{x,y}=2\alpha\mu_{x,y}$ for $x,y\in f^{-1}(b)$ and $v_{x,y}=2\beta\mu_{x,y}$ otherwise. This satisfies the constraint in the linear program for $\rec_\eps^{b}(f)$, and therefore witnesses that $\rec_\eps^{b}(f)\geq 2\alpha(1-\eps)\mu(f^{-1}(b))-2\beta\eps\mu(f^{-1}(\bar{b}))\geq \alpha(1-\eps)-\beta\eps$, since $\mu(f^{-1}(b))\geq 1/2$.
% \end{proof}
% 
% \begin{proof}[Proof of~\autoref{claim:non-dist-srec} (sketch)]
% The proof closely follows the lines of the proof of~\cite[Lemma 2]{JK10}, so we refer the reader to this reference for details.
% 
% For Item~1, let us consider an optimal point for $\srec_{\eps}^{b}(f)=k$. From the values $v_{x,y}$ and $w_{x,y}$, we will construct a function $g$ and a distribution $\mu$ such that $\mu(g^{-1}(b))\geq 1/2$, $\Pr_{(x,y)\leftarrow\mu}[f(x,y)\neq g(x,y)]<\delta$ and $\rec_\eps^{b,\mu}(g)\geq k$. We can assume without loss of generality that for any $(x,y)\in f^{-1}(\bar{b})$, we have $w_{x,y}=0$, and for any $(x,y)\in f^{-1}(b)$, we have either $v_{x,y}=0$ or $w_{x,y}=0$. We define the function $g$ as follows: $g(x,y)=f(x,y)$ iff $w_{x,y}=0$, and $g(x,y)\neq f(x,y)$ otherwise. We the introduce intermediate variables $v'_{x,y}$ such that $v'_{x,y}=v_{x,y}$ if $w_{x,y}=0$, and $v'_{x,y}=w_{x,y}$ otherwise. We then set $\alpha=\sum_{(x,y)\in g^{-1}(b)}v'_{x,y}$ and $\beta=\sum_{(x,y)\in g^{-1}(\bar{b})}v'_{x,y}$. Finally, we set $\mu_{x,y}=v'_{x,y}/(2\alpha)$ for $(x,y)\in g^{-1}(b)$ and $\mu_{x,y}=v'_{x,y}/(2\beta)$ for $(x,y)\in g^{-1}(\bar{b})$. It can then be shown that the function $g$ and the distribution $\mu$ satisfy the necessary conditions.
% 
% For Item~2, let $\mu$ be a distribution maximizing $\srec_{2\eps,\frac{\eps}{2}}^{b,\mu}(f)$ and $g$ be a function such that $\srec_{2\eps,\frac{\eps}{2}}^{b,\mu}(f)=\rec_{2\eps}^{b,\mu}(g)$ with $\mu(g^{-1}(b))\geq 1/2$ and $\Pr_{(x,y)\leftarrow\mu}[f(x,y)\neq g(x,y)]<\eps/2$. Finally, let $\alpha,\beta$ be an optimal point of the linear program~(\ref{eq:rec-dual}) for $\rec_{2\eps}^{b,\mu}(g)$. Note that we can assume without loss of generality that $g(x,y)\neq f(x,y)\Rightarrow f(x,y)=b$. Let us set $v_{x,y}=2\alpha\mu_{x,y}$ if $f(x,y)=g(x,y)=b$, $v_{x,y}=2\beta\mu_{x,y}$ if $f(x,y)=g(x,y)=\bar{b}$, and $v_{x,y}=0$ if $f(x,y)\neq g(x,y)$. Moreover, let us set $w_{x,y}=2\beta\mu_{x,y}$ if $f(x,y)\neq g(x,y)$, and $w_{x,y}=0$ otherwise. It can be shown that these values satisfy the constraint in the linear program for $\srec_{\eps}^{b}(f)$, and the corresponding objective value is at least $(1-2\eps)\alpha-2\eps\beta=\rec_{2\eps}^{b,\mu}(g)$.
% \end{proof}

 
\section{Proofs of Claims}
\label{app:claims}

\subsection{Claims about the single sampling experiment}



We will use the following lemma that appears in \cite{Bra11b}.
\begin{lemma}[\cite{Bra11b}]
\label{lem:typical}
For all $\tau, \nu, \Delta, \eps$, it holds that
$\tau(\Bad_\Delta(\tau, \nu)) \leq \frac{D(\tau \parallel \nu) + 1}{
  \Delta}$. 
\end{lemma}

\begin{proof}[\autoref{lem:single}]
We use the arguments first given in \cite{BW11} and prove the items in order.
\begin{enumerate}
\item \textbf{Probability Alice/Bob accepts.}  We do the
  analysis for Alice; the case for Bob is entirely symmetric.  We may
  write:
\begin{align*}
\Pr[\text{Alice accepts}] & = \sum_{u \in \calU}
\frac{1}{|\calU|} \frac{p_{\Al}(u)}{2^\Delta} q_{\Al}(u) 
 = \frac{1}{|\calU|2^\Delta} \sum_{u \in \calU} \nu_\Al(u) 
 = \frac{1}{|\calU|2^\Delta}
\end{align*}


\item \textbf{Probability of accepting.} First consider
  $u \notin B$.  For such $u$, if $\alpha \leq p_{\Al}(u)$
  then $\alpha \leq 2^\Delta q_{\Bo}(u)$ and also if $\beta \leq
  p_{\Bo}(u)$ then $\beta \leq 2^\Delta q_{\Al}(u)$.  Therefore we
  may write
  \begin{equation}
    \label{eq:notbad}
  \Pr[\text{Experiment outputs $u$}] = \frac{1}{|\calU|}
  \frac{p_{\Al}(u) p_{\Bo}(u)}{2^{2\Delta}} = \frac{\tau(u)}{|\calU|
    2^{2\Delta}}
  \end{equation}

  Furthermore, for any $u \in \calU$, we may write
  \begin{equation}
    \label{eq:allu}
    \Pr[\text{Experiment outputs }u] \quad = \quad \frac{1}{|\calU|2^{2\Delta}} \cdot
    \min\left\{ p_{\Al}(u), q_{\Bo}(u) 2^\Delta \right\} \cdot \min\left\{ p_{\Bo}(u), 
      q_{\Al}(u) 2^\Delta \right\} \quad \leq \quad
    \frac{\tau(u)}{|\calU|2^{2\Delta}}
  \end{equation}
  
  To prove the bounds on the probability of accepting, note that the
  upper bound follows from \autoref{eq:allu} because:
  $$\Pr[\exists u \in \calU,\ \text{Experiment outputs $u$}] = \sum_{u
    \in \calU} \Pr[\text{Experiment outputs $u$}] \leq \sum_{u \in
    \calU} \frac{\tau(u)}{|\calU|2^{2\Delta}} =
  \frac{1}{|\calU|2^{2\Delta}}$$ %
  The lower bound follows from \autoref{eq:notbad} since
  \begin{align*}
    \sum_{u \in \calU} \Pr[\text{Experiment outputs $u$}] & \geq \sum_{u
      \notin B} \Pr[\text{Experiment outputs $u$}] \\
    & = \sum_{u \notin B} \frac{\tau(u)}{ |\calU|2^{2\Delta}} \quad =
    \quad \frac{1 - \tau(B)}{|\calU|2^{2\Delta}} \quad = \quad \frac{1
      - \gamma}{|\calU|2^{2\Delta} }
  \end{align*}

\item \textbf{Statistical closeness of $\tau$ and $\tau'$.} Let $\eta$ denote the
  probability that the experiment is accepted.  From the
  previous point, we have that $\eta \in [ \frac{1 -
    \gamma}{|\calU|2^{2\Delta}}, \frac{1}{|\calU| 2^{2\Delta}}]$.  By
  the definition of statistical distance, it suffices to prove that:
  \begin{equation}
    \label{eq:stat}
    \forall S \subseteq \calU, \quad \tau(S) - \tau'(S) \leq \gamma
  \end{equation}

  We proceed by splitting the elements of $S$ based on whether they
  intersect $B$.
  \begin{align}
    \tau(S) - \tau'(S) & = \tau(S \cap B) - \tau'(S \cap B) + \tau(S \cap
    \oB)
    - \tau'(S \cap \oB) \nonumber\\
    & \leq \gamma + \tau(S \cap \oB) - \tau'(S \cap
    \oB) \label{eq:aosibz}
  \end{align}
  From \autoref{eq:notbad} we can deduce that $\tau'(S \cap \oB) =
  \frac{\tau(S \cap \oB)}{|\calU| 2^{2\Delta} \eta}$.  Therefore:
  \begin{align*}
    \tau(S \cap \oB) - \tau'(S \cap \oB) & = \tau(S \cap \oB) (1 -
    \tfrac{1}{|\calU| 2^{2\Delta} \eta})
  \end{align*}
  Since $\eta \leq \frac{1}{|\calU|2^{2\Delta}}$, we have that
  $(1 - \frac{1}{|\calU|2^{2\Delta} \eta}) \leq 0$.  Plugging this back
  into \autoref{eq:aosibz} we obtain \autoref{eq:stat}.
\end{enumerate}
\end{proof}

\subsection{Claims about the zero communication protocol}

 In the following, we will frequently use the fact that for all $p,
 \alpha \in [0, 1]$, it holds that $p(1 - \alpha) \geq p - \alpha$.

% Also, if $\Pr[f(X, Y) = b] \leq \beta$ then the compression lemma is trivially
% true.  So in the following let us assume that $\Pr[f(X, Y) = b] >  \beta$.
%\comm{Check if we still need something like this.}

\begin{proof}[Proof of \autoref{claim:compresspf}]
  We extend the arguments given in \cite{BW11} to prove the items of the claim in order.
  \begin{enumerate}
 

 \item By the definition of information complexity and the fact that mutual
    information is equal to the expectation of the divergence, we have that for $(X, Y)$ distributed according to
    $\mu$, 
    \begin{align*}
      \IC_\mu(\pi) & = I(X ; \Pi \mid Y) + I(Y ; \Pi \mid X) 
       = \Exp_{(x, y) \leftarrow (X,Y)} [D(\Pi_{x,y} \parallel \Pi_y) +
      D(\Pi_{x,y} \parallel \Pi_x)]
    \end{align*}
    This implies that $\Exp_{(x, y) \leftarrow (X,Y)} [D(\Pi_{x,y} \parallel
    \Pi_x)] \leq \IC_\mu(\pi)$, and since divergence is non-negative
    we have by Markov's inequality that
    $$\Pr_{(x, y) \leftarrow (X,Y)} [D(\Pi_{x,y} \parallel \Pi_x) > 8
    \IC_\mu(\pi) / \delta] \leq \delta / 8$$ %
    The same argument holds for $D(\Pi_{x,y} \parallel \Pi_y)$ and  by a
    union bound, we have $\Pr_{(X,Y)\sim \mu}[B_D] \leq \delta/4$.


  \item We may write:
    \begin{align*}
 \lefteqn{\Pr_{\alean}[B_C]}\\
 & = \Pr[\exists i \neq j \in
      [T]\text{ s.t. }i \in (\calA \cup \calB), j \in (\calA \cup \calB), h(i) = h(j) = r] \\
      & \leq \sum_{i \neq j \in [T]} \Pr[i \in (\calA \cup \calB) \wedge j \in (\calA \cup
      \calB) \wedge h(i) = h(j) = r ] \\
        & = \sum_{i \neq j} \Pr[i \in (\calA \cup \calB) ]  \Pr[ j \in (\calA \cup \calB)] 
         \Pr[h(i) = h(j) = r ]
      \\ 
      & \leq T^2 \frac{4}{(|\calU|2^\Delta)^2} \cdot \frac{1}{2^{2k}} \\
      & \leq \tfrac{\delta}{16} \cdot 2^{-(k + \Delta)}
    \end{align*}
    where we have used the independence between
    the trials and independence of the $h$ from the trials, as well as \autoref{step:alicebob}
    of \autoref{lem:single}.


  \item We have 
\[
   \Pr_{\alean}[G] 
    = \Pr[\calA\neq \varnothing] \cdot \Pr[G
   \mid  \calA\neq \varnothing ].
\]
 Observe that an element $i$ is in $\calA$ if and only if
    experiment $i$ is accepted by Alice.  By \autoref{step:alicebob}
    of \autoref{lem:single}, the probability of Alice aborting each
    experiment $i$ is $1 - \frac{1}{|\calU|2^{\Delta}}$.  Since the
    experiments are independent, the probability of Alice aborting
    all experiments is
    $$  \Pr[\calA = \varnothing ] = \left(1 - \tfrac{1}{|\calU|2^{\Delta}} \right)^T \leq e^{-
      \frac{T}{ |\calU| 2^\Delta}} \leq \delta / 8$$

We assume now that $\calA$ is non empty and we denote by $i$ its first element.
  \begin{align*}\Pr&[G \mid\calA\neq \varnothing ] \\
 &  = \Pr[h(i) = r \mid \calA\neq \varnothing ] \Pr[i \in \calB \mid  i \in \calA  \wedge h(i)=r \wedge \calA\neq \varnothing]
  \end{align*}
  
 % The condition $\neg B_E$ assures that $\calA$ is non-empty.
    For all $j$, the probability that $h(j) = r$ is exactly $2^{-k}$,
    in particular this holds for the first element of $\calA$.
   
    For any $(x, y) \notin B_D$, we have that $D(\Pi_{x,y} \parallel
    \Pi_x) \leq 8 \IC_\mu(\pi) / \delta$.  Let us say that a
    transcript is ``bad for Alice'' (resp. Bob) if it lies in the set
    $\Bad_\Delta(\Pi_{x,y}, \Pi_x)$ (resp. in the set
    $\Bad_\Delta(\Pi_{x,y}, \Pi_y)$.  Using \autoref{lem:typical},
    this implies that
    \begin{align*}
      \gamma_A & = \Pr[\Pi_{x,y} \text{ bad for Alice}]
      \leq \frac{\frac{8}{\delta} \IC_\mu(\pi) + 1}{\Delta} \leq
      \delta/4         \label{eq:naobnzp} \\
      \gamma_B & = \Pr[\Pi_{x,y} \text{ bad for Bob}]
      \leq \delta/4 %\label{eq:oiasdjf}
    \end{align*}
    It follows that $\gamma = \Pr[\Pi_{x,y} \text{ bad for Alice or
      Bob}] \leq \gamma_A + \gamma_B \leq \delta / 2$.

    By definition, for any $j$, experiment $j$ is accepted if and
    only if $j \in \calA \cap \calB$.  Therefore, $\forall j \in [T]$:
    \begin{align*}
      \Pr[j \in \calB \mid j \in \calA] & =
      \Pr[\text{experiment $j$ is accepted} \mid j \in \calA ] \\
      & = \frac{\Pr[\text{experiment $j$ is accepted} ]}{\Pr[j \in \calA ]} \\ 
      & \geq \frac{1-\gamma}{2^\Delta} %\label{eq:npaoih} 
\\
      & \geq \frac{1-\frac{\delta}{2}}{2^\Delta}
    \end{align*}
    where we used \autoref{step:alicebob} and
    \autoref{step:nofail} of \autoref{lem:single}, and
    the fact that $\neg B_D$ implies that $\gamma \leq \delta/4$.

    Also, observe that by the definition of the protocol, the choice
    of $h$ and $r$ are completely independent of the experiments.
    Therefore we may add the condition that $h(j) = r$ without
    altering the probability. Since $j \in \calA$ implies $\calA\neq \varnothing$, we can add this condition too.
    Finally, we use this with $j=i$.
We conclude 
\[
 \Pr_{\alean}[G] \geq (1-\delta/8) \frac{1-\frac{\delta}{4}}{2^{k+\Delta}} \geq  \frac{1-\frac{5\delta}{8}}{2^{k+\Delta}}
\]

  \item As in the previous point we will use the fact that:
  \begin{align*}
\Pr_{\alean}[G ] & = \Pr[\calA\neq \varnothing] \Pr[h(i) = r\mid\calA\neq \varnothing ] \Pr[i \in \calB \mid i \in \calA  \wedge h(i)=r \wedge \calA\neq \varnothing]\\
&\leq \Pr[h(i) = r\mid\calA\neq \varnothing ] \Pr[i \in \calB \mid i \in \calA  \wedge h(i)=r \wedge \calA\neq \varnothing]
  \end{align*}
As before the first factor is exactly $2^{-k}$ for any $i$.
  We may also write:
    \begin{align*}
      \Pr[i \in \calB \mid i \in \calA ] & =
      \Pr[\text{experiment $i$ is accepted} \mid i \in \calA ] \\
      & = \frac{\Pr[\text{experiment $i$ is accepted}]}{\Pr[i \in \calA]} \\
      & \leq \frac{1}{2^\Delta},
    \end{align*}
where we used  \autoref{step:alicebob} and
    \autoref{step:nofail} of \autoref{lem:single}.
    As with the previous point, adding the conditions $h(i) = r$ and $\calA\neq\varnothing$ does
    not affect the probabilities.
    
  \item The distribution of $\Pi'_{x,y}$ conditioned on not aborting
    \emph{and} no collision is simply the distribution of the output
    of a single experiment, and we know from the facts about the
    single experiment (\autoref{lem:single}) that this is close to
    $\Pi_{x,y}$.  We wish to conclude that $\Pi'_{x,y}$ conditioned
    \emph{only} on not aborting is also close to $\Pi_{x,y}$.  The
    following lemma allows us to do this by using the fact that the
    probability of collision is small:
  \begin{lemma}
    \label{lem:conditional}
    Let $\Pi$ and $\Pi'$ two distributions taking output in a common
    universe. We let $\Pi'_E$ denote the distribution $\Pi'$
    conditioned on $E$.  Let $E$, $F$, and $H$ three events in
    the underlying probability space of $\Pi'$ where $E \subseteq H$
    and $(H - E) \subseteq F$ and satisfying:
  \begin{itemize}
  \item $\Pr_{\Pi'}[F] \leq \delta_F$
  \item $\Pr_{\Pi'}[H] \geq \delta_H$
  \item $|\Pi'_E - \Pi| \leq c$
  \end{itemize}
  Then it holds that $|\Pi'_H - \Pi| \leq c + \frac{\delta_F}{\delta_H}$
  \end{lemma}
  \begin{proof}
    For shorthand, for any event $E$ let us write $\Pi'_H(E) =
    \Pr_{\Pi'}[E \mid H]$, and similarly for $\Pi'(E)$ and $\Pi(E)$.
    For a set $S$ in the support of $\Pi'$ and $\Pi$, we let $S$ also
    denote the event that the value of the random variable is in $S$.

    It suffices to prove that, for all subsets $S$ in the union of the
    supports of $\Pi$ and $\Pi'_H$, it holds that $\Pi'_H(S) - \Pi(S)
    \leq c + \frac{\delta_F}{\delta_H}$.  To show this, we may write:
    \begin{align*}
      \Pi'_H (S) - \Pi(S) &  = \frac{\Pi'(H \cap S)}{\Pi'(H)} - \Pi(S)
      \\
      & \leq  \frac{\Pi'(E \cap S) + \Pi'((H-E) \cap S)}{\Pi'(H)} - \Pi(S) \\
      & \leq  \frac{\Pi'(E)(c+ \Pi(S)) + \Pi'(F)}{\Pi'(H)} -\Pi(S)
    \end{align*}
    because $(H-E) \subset F$ and $|\Pi'_E - \Pi| \leq c$.  Because $E
    \subset H$, we can conclude that:
    $$ \Pi'_H(S) - \Pi(S) \leq \frac{\Pi'(F)}{\Pi'(H)} + c \leq c +
    \frac{\delta_F}{\delta_H}$$  
 \end{proof}
   
   We apply this lemma with $\Pi = \Pi_{x,y}$, $\Pi' = \Pi'_{x,y}$,
   $E= G-B_C$, $F = B_C$, and $H$ the event that $\Pi'_{x,y} \neq
   \bot$.  We calculate $c$, $\delta_F$ and $\delta_H$:
  \begin{itemize}
  
   \item Since $h$ and $r$ are completely independent of the actual
     experiments themselves, it holds that the distribution of
     $\Pi'_{x,y}$ conditioned on $G-B_C$ is identical to the output of
     a single experiment (\autoref{alg:experiment}). Since $(x, y)
     \notin B_D$, the measure of the bad set $\Bad_\Delta(\Pi_{x,y},
     \Pi_y) \cup \Bad_\Delta(\Pi_{x,y}, \Pi_x)$ is bounded by
     $\delta/2$.  We apply \autoref{step:stat} of \autoref{lem:single}
     to deduce that $| \Pi_{x,y} - \Pi'_{x, y,E} | \leq \delta/2 = c$.
    
   \item For all $(x, y) \notin B_D$, since the probability of $H$ is
     at least the probability of $G - B_C$, we have that:
     \begin{align} 
       \delta_H = \Pr_{\alean}[H] = \Pr_{\alean}[\pi'(x, y) \neq \bot]
       \geq (1 - \frac{11\delta}{16})
       2^{-(k+\Delta)}\label{eq:lowerbound}
     \end{align}
     The last inequality follows from \autoref{item:collision} and
     \autoref{item:gooda} of \autoref{claim:compresspf}.
   
   \item From \autoref{item:collision}, we know that $\delta_F =
     \Pi_{x,y}(B_C) \leq \frac{\delta}{16} \cdot 2^{-(k+\Delta)}$.
   
 \end{itemize}
 
 Therefore, \autoref{lem:conditional} implies that:
 $$| \Pi_{x,y} - \Pi^{' \neq \bot}_{x, y} | \leq \delta/2 +
 \frac{\delta}{16(1- \frac{11\delta}{16})} \leq \delta/2 + \delta/5 <
 3\delta/4$$ 
 where we use the assumption that $\delta \leq 1$.
\end{enumerate}
\end{proof}


\section{Applications}
\subsection{Vector in Supspace problem}
\label{app:VSP}

Klartag and Regev's lower bound is based on the following lemma:
\begin{lemma}[\cite{KR11}]\label{lem:klartag-regev}
Let $f=\VSP_{0,n}$, $\calX$ and $\calY$ denote Alice and Bob's input sets for $f$, $\sigma$ be the uniform distribution over $\calX\times\calY$ and $\sigma_b$ be the uniform distribution over $f^{-1}(b)$. There exist universal constants $C$ and $\gamma$ such that, for any rectangle $R$ and any $b\in\zo$, we have:
\begin{align*}
 \sigma_b(R\cap f^{-1}(b))\geq 0.8\sigma(R)-C\exp(-\gamma n^{1/3}).
\end{align*}
\end{lemma}

We show that this implies that $\log\bprt_\eps(\VSP_{0,n})=\Omega(n^{1/3})$. Note that since the input set of $\VSP_{0,n}$ is continuous, we need to extend the definition of the relaxed partition bound to the case of a continuous input set, but this follows naturally by replacing summation symbols by integrals.
\begin{lemma}
There exist universal constants $C$ and $\gamma$ such that for any $\eps$,
$\bprt_\eps(\VSP_{0,n})\geq\frac{1}{C}(0.8-2.8\eps)\exp (\gamma n^{1/3})$.
\end{lemma}
\begin{proof}
Let $\mu=\frac{\sigma_0+\sigma_1}{2}$, which satisfies $\mu(f^{-1})=1$, \ie $\mu$ only has support on valid inputs. Then, Lemma~\ref{lem:klartag-regev} implies that for any rectangle $R$ and any $b\in\zo$, we have
\begin{align*}
 2\mu(R\cap f^{-1}(b \oplus 1))\geq 0.8\sigma(R)-C\exp(-\gamma n^{1/3}).
\end{align*}
Since $\mu$ only has support on $f^{-1}$ and $f$ is Boolean, we have $\mu(R)=\mu(R\cap f^{-1}(b))+\mu(R\cap f^{-1}(b\oplus 1))$, so that the inequality can be rewritten as
\begin{align*}
 2\mu(R)-2\mu(R\cap f^{-1}(b))\geq 0.8\sigma(R)-C\exp(-\gamma n^{1/3}).
\end{align*}
Setting $t=\frac{\exp(\gamma n^{1/3})}{C}$, we have that:
\begin{align*}
 t\cdot \left( 2\mu(R\cap f^{-1}(b))+0.8\sigma(R)-2\mu(R)\right) \leq 1
\end{align*}

We now construct a feasible point for the dual formulation of $\bprt_\eps(f)$ given in \autoref{claim:bprt-lp} by setting $\alpha(x,y)=2t\mu(x,y)$ for $(x,y)\in f^{-1}$ and $\alpha(x,y)=0.8t\sigma(x,y)$ otherwise; and $\beta(x,y)=2t\mu(x,y)-0.8t\sigma(x,y)$ for $(x,y)\in f^{-1}$, and $\beta(x,y)=0$ otherwise. Note that for $(x,y)\in f^{-1}$, we have $\mu(x,y)=\sigma(x,y)/\sigma(f^{-1})\geq\sigma(x,y)$, hence all these values are positive. By the previous inequality, we also have
\begin{align*}
 \int_{R \cap f^{-1}(b)} \alpha(x,y) dxdy+ \int_{R \setminus f^{-1}}
\alpha(x,y) dxdy- \int_{R}\beta(x,y) dxdy \leq 1
\end{align*}
for any $R,b$, therefore this is a valid feasible point. Finally, the corresponding objective value is
\begin{align*}
  \int_{\calX\times\calY} (1 - \eps) \alpha(x,y) dxdy-
  \int_{\calX\times\calY} \beta(x,y) dxdy &=t\left( (1-\eps)2\mu(f^{-1})+(1-\eps)0.8(1-\sigma(f^{-1}))-2\mu(f^{-1})+0.8\sigma(f^{-1})\right)\\
&=t(0.8-2.8\eps+0.8\eps\sigma(f^{-1}))\\
&\geq t(0.8-2.8\eps).
\end{align*}
\end{proof}
Finally, let us note that we can construct a zero-communication protocol for $\VSP_{0,n}$ by first rounding off the inputs, and then applying a zero-communication protocol for $\tVSP_{\theta,n}$. This means that we can turn a feasible point for 
the primal form of $\bprt_\eps(\tVSP_{\theta,n})$ (given in \autoref{claim:bprt-lp}) into a feasible point for $\bprt_\eps(\VSP_{0,n})$ with the same objective value, so that $\bprt_\eps(\VSP_{0,n})\leq\bprt_\eps(\tVSP_{\theta,n})$. 

Therefore, the previous lemma together with \autoref{thm:mainthm} imply that $IC_\eps(\tVSP_{\theta,n})=\Omega(n^{1/3})$ and also \autoref{VSP}.



\subsection{Gap Hamming Distance}
\label{app:GHD}


Let us recall the linear program for the rectangle bound
as given by Jain and Klauck~\cite{JK10}.
\begin{theorem}
For any function $f$, 
and $\epsilon, \delta \beta>0$
if a distribution on the inputs $\mu$ is such that
$$\mu(R) > \beta \implies \mu(R\cap f^{-1}(z))>\delta \mu(R\cap f^{-1}(1-z))$$then
$$2^{R_\epsilon(f)} \geq \frac{1}{\beta}(\mu(f^{-1}(z)) - \frac{\epsilon}{\delta}).$$
\end{theorem}

We can derive the general corruption bound as used by Sherstov 
by giving a feasible solution to the 
dual of the linear program by Jain and Klauck.  
In the dual form, $\rect_\eps^{z,\mu}(f)$ is defined as 
\begin{align}
\rect_\eps^{z,\mu}(f)=\max_{\alpha_{x,y}\geq 0} & 
	(1 - \eps)\sum_{(x,y)\in f^{-1}(z)} \alpha_{x,y} 
	- \eps\sum_{(x,y)\in f^{-1}\setminus f^{-1}(z)} \alpha_{x,y} \\
\forall R, & \quad 
	\sum_{(x,y)\in R\cap f^{-1}(z)} \alpha_{x,y} 
	- \sum_{(x,y)\in R\cap(f^{-1}\setminus f^{-1}(z))} \alpha_{x,y} \leq 1.
\end{align}

Consider the following assignment for $\rect_\eps^{-1, \mu}$, where
$\mu$ is the distribution over the inputs in the theorem.
Let $\Delta_{-1} = \frac{1}{\beta}$ and  
$\Delta_{+1} = \frac{1}{\delta}\Delta_{-1}$, and
 $ \alpha_{x,y} = \Delta_{f(x,y)} \mu(x,y).$
	
Since the function is boolean,  $f^{-1}\setminus f^{-1}(z) = f^{-1}(+1)$.
The left hand side of the constraint now reads:
\begin{eqnarray*}
	\lefteqn{\sum_{(x,y)\in R\cap f^{-1}(-1)} \alpha_{x,y} 
		- \sum_{(x,y)\in R\cap f^{-1}(+1)} \alpha_{x,y}} \\
&=&   \Delta_{-1}\mu( R\cap f^{-1}(-1)) -  \Delta_{+1} \mu(R\cap f^{-1}(+1)) \\
&=&   \Delta_{-1}\mu( R\cap f^{-1}(-1)) - \frac{1}{\delta}\Delta_{-1}  \mu(R\cap f^{-1}(+1)).
\end{eqnarray*}
If  $\mu(R) \leq \beta$, then  $\Delta_{-1}\mu( R\cap f^{-1}(-1)) \leq 1 $, and 
the constraint is verified.

If $\mu(R) > \beta$, then we apply the hypothesis.
\begin{eqnarray*}
 \lefteqn{\Delta_{-1}\mu( R\cap f^{-1}(-1)) - \frac{1}{\delta}\Delta_{-1}  \mu(R\cap f^{-1}(+1))}\\
&\leq& \Delta_{-1}\mu( R\cap f^{-1}(-1) ) - \frac{1}{\delta}\Delta_{-1}  \mu(R\cap f^{-1}(+1))\\
&\leq& \Delta_{-1}\mu( R  \cap f^{-1}(-1)) - \Delta_{-1}  \mu(R \cap f^{-1}(-1))\\
&\leq& 1
\end{eqnarray*}
and the constraint is also verified in this case.

Letting $\mu= \mu(f^{-1}(-1))$, the value of the objective function is
\begin{eqnarray*}
\lefteqn{(1 - \eps)\Delta_{-1}\mu 
	- \eps  \Delta_{+1}\mu(f^{-1}(+1)) }\\
&=& (1 - \eps)\Delta_{-1}\mu - \frac{\eps}{\delta}\Delta_{-1} \mu(f^{-1}(+1))\\
&\geq &  (1 - \eps)\Delta_{-1}\mu -\frac{\eps}{\delta} \Delta_{-1}  (1-\mu)\\
&=& \Delta_{-1} (  (1 - \eps)\mu - \frac{\eps}{\delta}  (1-\mu))\\
&\geq& \frac{1}{\beta} (\mu-\frac{\eps}{\delta})
\end{eqnarray*}
This shows that the corruption bound is at most 
$\rect_\eps^{z,\mu}$, so any lower bound on the corruption
bound is also a lower bound on $\rect_\eps^{z,\mu}$.




==> macros.tex <==
\def\DaveMacros{1}

\providecommand{\size}{\mathsf{SIZE}}
\providecommand{\remove}[1]{}
\providecommand{\parens}[1]{\left(#1\right)}

\providecommand{\ie}{\emph{i.e.}{} }
\providecommand{\eg}{\emph{e.g.}{} }

\providecommand{\Enc}{\mathrm{Enc}}
\providecommand{\Dec}{\mathrm{Dec}}
\providecommand{\supp}{\mathrm{supp}}
\providecommand{\Exp}{\mathbb{E}}
\providecommand{\implique}{\Rightarrow}
\providecommand{\dans}{\rightarrow}
\providecommand{\equivaut}{\Leftrightarrow}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\sign}{\mathrm{sign\ }}
\providecommand{\vspan}{\mathrm{span}}
\providecommand{\abs}{\mathrm{abs\ }}
\providecommand{\Tr}{\mathrm{Tr}}
\providecommand{\eps}{\varepsilon}
\providecommand{\zo}{\{0, 1\}}



\providecommand{\SAT}{\mathsf{SAT}}
\providecommand{\UNSAT}{\mathsf{UNSAT}}
\providecommand{\coAM}{\mathbf{coAM}}
\providecommand{\P}{\mathbf{P}}
\providecommand{\BPP}{\mathbf{BPP}}
\providecommand{\RP}{\mathbf{RP}}
\providecommand{\ZK}{\mathbf{ZK}}
\providecommand{\SZK}{\mathbf{SZK}}
\providecommand{\CZK}{\mathbf{CZK}}
\providecommand{\NP}{\mathbf{NP}}
\providecommand{\coNP}{\mathbf{coNP}}
\providecommand{\bPi}{\mathbf{\Pi}}
\providecommand{\bSigma}{\mathbf{\Sigma}}
\providecommand{\SPACE}{\mathbf{SPACE}}
\providecommand{\NSPACE}{\mathbf{NSPACE}}
\providecommand{\NL}{\mathbf{NL}}
\renewcommand{\L}{\mathbf{L}}
\providecommand{\APSPACE}{\mathbf{APSPACE}}
\providecommand{\PSPACE}{\mathbf{PSPACE}}
\providecommand{\IP}{\mathbf{IP}}
\providecommand{\ACC}{\mathbf{ACC}}


\providecommand{\co}[1]{\mathbf{co#1}}
\providecommand{\PCP}[2]{\mathbf{PCP}(#1, #2)}
\providecommand{\drawn}[1]{\stackrel{#1}{\leftarrow}}
\providecommand{\drawnr}{\drawn{R}}
\renewcommand{\Pr}{\mathop{\mathrm{Pr}}}

\providecommand{\Ext}{\mathrm{Ext}}

\def\FullBox{\hbox{\vrule width 8pt height 8pt depth 0pt}}


\def\qed{\ifmmode\qquad\FullBox\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\FullBox
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}



\newenvironment{piecewise}{\left\{\begin{array}{l@{,\ }l}}
{\end{array}\right.}

\makeatletter
\@addtoreset{equation}{section}
\makeatother
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}


